Human-Data Interaction: The Human Face of the Data-Driven Society

The increasing generation and collection of personal data has created a complex ecosystem, often collaborative but sometimes combative, around companies and individuals engaging in the use of these data. We propose that the interactions between these agents warrants a new topic of study: Human-Data Interaction (HDI). In this paper we discuss how HDI sits at the intersection of various disciplines, including computer science, statistics, sociology, psychology and behavioural economics. We expose the challenges that HDI raises, organised into three core themes of legibility, agency and negotiability, and we present the HDI agenda to open up a dialogue amongst interested parties in the personal and big data ecosystems.

==> challenges.tex <==
\section{Challenges}
\label{s:call}

What are the implications of HDI? How should researchers engage with HDI? The following existing domains clearly intersect with HDI; no doubt there are many others.

%generally think i'd structure each topic as:
%- motivation- why important
%- examples- what research is going on
%- future- what looks like being the future capability here

\textbf{HCI \& Data Visualisation.} As discussed above, HCI clearly overlaps with HDI, particularly in topics relating to data visualisation. Many of the concepts and datasets that motivate the need for HDI are rather abstract: enabling subjects to interact naturally with their data and the algorithms processing them is an important goal. Some existing work in this space uses embodied allegories to support the design of meaningful Embodied Interactions~\cite{embodiedHDI,Cafaro:2012:UEA:2370216.2370309}.

Interaction with data also needs an understanding of the alignment of incentives: appropriate and smart data visualisations may reveal aspects of the incentive models, this kind of visualisation should be coupled with field investigations that are sociologically grounded and use ethnographic methods. Examples include challenges faced by personal data and Quantified Self app developers in presenting the vast amount of data collected about a single individual~\cite{chi_vis_chal}. 


\textbf{Sensing and Analytics.} 

For industry, perhaps the most important aspect of personal data use is analytics. As new sources of \textit{Big Data} arise, characterised by volume, variety, and velocity~\cite{bigdata3v}, new analytics methods will arise, with resultant effects for how users should interact and interpret these data. One growing source of such data is the Internet of Things (IoT), which will create increasing amounts of ambient data from our urban environment~\cite{Zaslavsky}. Recent interest in the \emph{Quantified Self} also relies on data collation and analytics about physical activity, dietary data, sleep patterns, and so forth. 

Within this space, a number of challenges lie, including understanding the effects, reaction and individual behaviours changes when dealing with analytics outcomes, epistemology and ontology of analytics, dependencies and provenance  of data sources, and possibility of aggregation at granularity level that hide individual information (see ~\cite{privalytics}). 


\textbf{Privacy \& Security.}

Outdated regulation, coupled with cultural differences in service provision and online behaviour, have resulted in a wave of strong user reactions in response to political events and industrial developments in the \emph{Big Data Analytics} era. In reaction to this trend, individuals, governments, privacy advocates, industry, and regulators have been fiercely fighting their corners concerning the collection, use, trade, and retention of personal information. For example, the UK has seen strong reactions on social media to plans on scanning customers' faces at supermarkets and selling the images to advertisers~\cite{hawkes:tesco}.

Increasing pervasive data collection and third party tracking by advertisers on websites and OSNs (~\cite{Krishnamurthy,MarjanTMA,Butkiewicz:webcomplexity}), introduce new challenges to the privacy of personal data. Some of these are centred around the individual. Do individual's perceived data values change from day to day? Would they react to dynamic, on-going consent processes? Will they adopt privacy mechanisms such as differential privacy~\cite{diffpriv}, or privacy-preserving profiling and advertising schemes such as Adnostic~\cite{adnostic}, MobiAd~\cite{mobiad}, or PrivAd~\cite{guha.hotnets09}? Other challenges are centred around the services and organisations which focus on collecting and analysing personal data. How will they deal with the issue of contextual privacy, ethics, informed consent and its meaning~\cite{literatin,ioannidis:oxymoron,nissenbaum:integrity}? Will they adhere to self-regulation and  trust certification schemes?\tnhh{ref?}


\textbf{Open Data \& Knowledge}

The power of open data, open knowledge, and open innovation is now advocated for by a number of independent organisations.\footnote{e.g., \url{http://www.datasociety.net/}, \url{http://okfn.org}, and \url{http://theodi.org}} The objective of these efforts is to free individuals and the Web from echo chambers and filter bubbles~\cite{pariser:filter}, and empower individuals through transparent access and audit of governments and various organisations. Examples include Open Data and public health\footnote{\url{http://openmhealth.org}}, OpenStreetMap\footnote{\url{http://www.openstreetmap.org/}}, and open reports of crime data\tnhh{ref}. The general hope is that publishing data will encourage making it participatory and accessible. However releasing data to the public needs care and foresight into usage, correlation, and reputation side effects. Availability of certain crime data about a specific neighbourhood may intact reinforce that area as a hub. Hence the open data challenge is still an unresolved one from an HDI perspective. \hamed{I was thinking more about drugs and prostitution, that for example everyone knew you;d go to kings x for prostitutes and camden for drugs...}


\textbf{Social Psychology.} 

Individuals' decision making can be manipulated in many ways, e.g.,~by altering the choices available and the order in which they are presented~\cite{nudge}. Interaction with online content is also affected by the way in which information is presented. Even in population-scale Big Data industries, the human factors of judging ambiguities and cross-referencing terms across social and cultural boundaries remain key elements~\cite{nytimesAlgorithms}. Other examples of tension between data availability and actions include online reputation and one's reflection from that reflection\tnhh{what does ``reflection from reflection'' mean?}, with certain context and empathy. The availability of data about an individual online can certainly change the way their public image is perceived by others, hence affecting their own behaviour\tnhh{``certainly'' is very strong so references are needed.}. 

Other example of the feedback loop between behaviour and data include the accuracy of keyword popularity prediction algorithms. For example, Google has used search term analytics to work out the way a flu epidemic is evolving, although such approaches are also subject to false positives due to hype bias in the news resonating and amplifying observed effects~\cite{googleflu}. The challenge is to apply the tools of fields such as social psychology and computational linguistics to better understand these effects, on-line and at scale~\cite{linguistics-journal}.


\textbf{Behavioural Economics.}

The increasing rate of \emph{Social Computing} application, aiming to convert data, to information, and ultimately to knowledge is also an increasingly important challenge in utilising individuals' data. This bottom-up knowledge productions sees data as a \textit{potential capacity}; in most cases we don't know what the context is or what it is useful for, but we are collecting it in the belief that it may have some future value or utility. This includes many of the Quantified Self applications. 
\tnhh{not sure that I see the relationship between social computing and behavioural economics. If we want to discuss social computing, then we ought to mention~\cite{bernstein:problem}}

We also need to understand how recent behavioural targeting advances in advertising have affected the personal data collection ecosystem. There currently is disproportionate economic power in the hands of the data aggregators acting as data brokers and mediators for the users. It may be possible to enable an ecosystem using economic value models for utilisation of personal data~\cite{hotplanet13,Gill:2013:BPF:2504730.2504768} and marketplaces~\cite{DBLP:journals/corr/abs-1205-0030}.

\textbf{Community and Culture}

Increasingly it is important to understand the cultural differences and similarities,  contexts differences. ownership definitions, and approaches to use, release, and distribution of personal data in different communities and cultures. There are often differences between one's personal, local, national, global image, reputation, and behaviour offline and online, from driving behaviour to mobile phone usage, energy usage, and online shopping. These lead to challenges in creating applications using individuals data or providing behaviour nudged and feedback based on collected data. 



%% \if 0

%Access to the Internet is increasingly seen as a human right~\cite{wicker:access}. The Internet's open, non-discriminatory shared nature has thus been of central interest to a number of advocacy groups. Changes in access to data often cause Internet activism, sometimes leading to political and regulatory change, e.g.,~the 2013 ITU voting case on Internet Governance~\cite{mccullagh:itu}. 


%% \fi

